On the Tool Manipulation Capability of Open-source Large Language Models

Recent studies on software tool manipulation with large language models (LLMs) mostly rely on closed model APIs. The industrial adoption of these models is substantially constrained due to the security and robustness risks in exposing information to closed LLM API services. In this paper, we ask can we enhance open-source LLMs to be competitive to leading closed LLM APIs in tool manipulation, with practical amount of human supervision. By analyzing common tool manipulation failures, we first demonstrate that open-source LLMs may require training with usage examples, in-context demonstration and generation style regulation to resolve failures. These insights motivate us to revisit classical methods in LLM literature, and demonstrate that we can adapt them as model alignment with programmatic data generation, system prompts and in-context demonstration retrievers to enhance open-source LLMs for tool manipulation. To evaluate these techniques, we create the ToolBench, a tool manipulation benchmark consisting of diverse software tools for real-world tasks. We demonstrate that our techniques can boost leading open-source LLMs by up to 90% success rate, showing capabilities competitive to OpenAI GPT-4 in 4 out of 8 ToolBench tasks. We show that such enhancement typically requires about one developer day to curate data for each tool, rendering a recipe with practical amount of human supervision.

==> tables/typical_errors.tex <==
\begin{table}[]
\centering
\caption{Typical Errors}
\label{tab:examples}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{@{}c|l@{}}
\toprule
    Prompt      & \begin{tabular}[c]{@{}l@{}}\# Get the weather forecast data in \{zipcode\} area\\ curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=\{zipcode\}\&appid=\{API\_KEY\}\{optional\_params\}'\\ \\ Given this API, tell me the temperature for the upcoming week in zip code 11962?\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\
\cmidrule(lr){1-2}
Expected results & curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&appid=\{API\_KEY\} \\
\midruleWrong 
Verbosity     & \begin{tabular}[c]{@{}l@{}}To get the temperature for the upcoming week in zip code 11962, you need to replace \{zipcode\} with 11962 and \{API\_KEY\} with \\your actual API key. You can also add optional parameters like units (metric or imperial) to get the temperature in Celsius or Fahrenheit. \\ Here's an example using the metric system:\\ \\ ```bash\\ curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&appid=YOUR\_API\_KEY\&units=metric | jq -r '.list[].main.temp''\\ ```\\ \\ Replace YOUR\_API\_KEY with your actual API key. This command will return a JSON object containing the weather forecast data \\ for the upcoming week in the 11962 area. You can then parse the JSON object to extract the temperature information for each day.\end{tabular} \\
% \midrule
% llama-30b & \textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n\textbackslash n                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    \\
% \midrule
% neox-20b  & \begin{tabular}[c]{@{}l@{}}You can use the following code:\\ import requests\\ \\ zipcode = '11962'\\ api\_key = 'your\_api\_key'\\ \\ url = 'https://api.openweathermap.org/data/2.5/forecast?zip=\{zipcode\}\&appid=\{api\_key\}'\\ \\ response = requests.get(url.format(zipcode=zipcode, api\_key=api\_key))\\ \\ print(response.json())\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                           \\
\cmidrule(lr){1-2}
Wrong API   & \begin{tabular}[c]{@{}l@{}} curl -X GET 'https://api.openweathermap.org/data/2.5/{\color{red}\textbf{air\_pollution}}?city=11962\&appid=\{API\_KEY\}\{optional\_params\}'\end{tabular}         \\
\cmidrule(lr){1-2}
Wrong Args.   & \begin{tabular}[c]{@{}l@{}}curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?{\color{red}\textbf{city}}=11962\&appid=\{API\_KEY\}\{optional\_params\}'\end{tabular}         \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}



% \begin{table}[]
% \centering
% \caption{Examples}
% \label{tab:all_models}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{@{}l|l|l@{}}
%           & \begin{tabular}[c]{@{}l@{}}\# Get the weather forecast data in \{zipcode\} area\\ curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=\{zipcode\}\&appid=\{API\_KEY\}\{optional\_params\}'\\ \\ Given this API, tell me the temperature for the upcoming week in zip code 11962? Answer in shell command only\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        & \begin{tabular}[c]{@{}l@{}}\# Get the weather forecast data in \{zipcode\} area\\ curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=\{zipcode\}\&appid=\{API\_KEY\}\{optional\_params\}'\\ \\ Given this API, tell me the temperature for the upcoming week in zip code 11962?\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\
% Chat-gpt  & \begin{tabular}[c]{@{}l@{}}Sure, here's the shell command to get the temperature for the upcoming week in zip code 11962 using the OpenWeatherMap API:\\ \\ curl -s 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&units=imperial\&appid=\{API\_KEY\}' | jq '.list{[}{]}.main.temp'\\ This command uses curl to send a GET request to the OpenWeatherMap API with the zip parameter set to 11962, the units parameter set to imperial (to get the temperature in Fahrenheit), and the appid parameter set to your API key.\\ \\ The output of this command is piped to jq, which is a command-line JSON processor. The jq expression .list{[}{]}.main.temp extracts the temp field from the main object in each item in the list array of the JSON response.\\ \\ The output will be the temperature values for the upcoming week at 3-hour intervals, so you'll get 56 temperature values in total.\end{tabular} & \begin{tabular}[c]{@{}l@{}}To get the temperature for the upcoming week in zip code 11962, you can make the following cURL request, replacing \{API\_KEY\} with your OpenWeatherMap API key:\\ \\ curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&appid=\{API\_KEY\}\&units=imperial'\\ This request will return a JSON response that includes the weather forecast data for the next five days, with temperature values in Fahrenheit. You can parse the JSON response to extract the temperature values for each day.\end{tabular}                                                                                                                                                                                                       \\
% gpt-4     & curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&appid=\{API\_KEY\}\&units=imperial'                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                    & \begin{tabular}[c]{@{}l@{}}To get the temperature for the upcoming week in zip code 11962, you need to replace \{zipcode\} with 11962 and \{API\_KEY\} with your actual API key. You can also add optional parameters like units (metric or imperial) to get the temperature in Celsius or Fahrenheit. Here's an example using the metric system:\\ \\ ```bash\\ curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&appid=YOUR\_API\_KEY\&units=metric'\\ ```\\ \\ Replace YOUR\_API\_KEY with your actual API key. This command will return a JSON object containing the weather forecast data for the upcoming week in the 11962 area. You can then parse the JSON object to extract the temperature information for each day.\end{tabular} \\
% llama-30b & \textless{}empty\textgreater{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                  & \textless{}empty\textgreater{}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\
% neox-20b  & \begin{tabular}[c]{@{}l@{}}You can use the following command:\\ curl -s 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&appid=\textless{}API\_KEY\textgreater{}\&units=metric\&cnt=7' | grep -oP '(?\textless{}=temp\textbackslash{}s*=\textbackslash{}s*)\textbackslash{}d+(?=\textbackslash{}s*C)'\\ \\ The output is:\\ \\ 25\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      & \begin{tabular}[c]{@{}l@{}}You can use the following code:\\ import requests\\ \\ zipcode = '11962'\\ api\_key = 'your\_api\_key'\\ \\ url = 'https://api.openweathermap.org/data/2.5/forecast?zip=\{zipcode\}\&appid=\{api\_key\}'\\ \\ response = requests.get(url.format(zipcode=zipcode, api\_key=api\_key))\\ \\ print(response.json())\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                           \\
% codegen   & curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&appid=\{API\_KEY\}\{optional\_params\}'                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                & \begin{tabular}[c]{@{}l@{}}\# Get the weather forecast data in zip code 11962\\ curl -X GET 'https://api.openweathermap.org/data/2.5/forecast?zip=11962\&appid=\{API\_KEY\}\{optional\_params\}'\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      
% \end{tabular}
% \end{adjustbox}
% \end{table}
